NADI 2024: The Fifth Nuanced Arabic Dialect Identification Shared Task

We describe the findings of the fifth Nuanced Arabic Dialect Identification Shared Task (NADI 2024). NADI's objective is to help advance SoTA Arabic NLP by providing guidance, datasets, modeling opportunities, and standardized evaluation conditions that allow researchers to collaboratively compete on pre-specified tasks. NADI 2024 targeted both dialect identification cast as a multi-label task (Subtask~1), identification of the Arabic level of dialectness (Subtask~2), and dialect-to-MSA machine translation (Subtask~3). A total of 51 unique teams registered for the shared task, of whom 12 teams have participated (with 76 valid submissions during the test phase). Among these, three teams participated in Subtask~1, three in Subtask~2, and eight in Subtask~3. The winning teams achieved 50.57 F\textsubscript{1} on Subtask~1, 0.1403 RMSE for Subtask~2, and 20.44 BLEU in Subtask~3, respectively. Results show that Arabic dialect processing tasks such as dialect identification and machine translation remain challenging. We describe the methods employed by the participating teams and briefly offer an outlook for NADI.

==> sections/rw.tex <==
%======================== DID ==============================
%papers I couldn't access:
%https://ieeexplore.ieee.org/abstract/document/10349904
%https://ieeexplore.ieee.org/abstract/document/10479320
%https://ieeexplore.ieee.org/abstract/document/10085647
%excluded:
%https://www.scirp.org/pdf/jsea_2023072811195844.pdf
%other papers to possibly cite for 2023-2024 (weak veunues):
%text: Arabic Regional Dialect Identification (ARDI) using Pair of Continuous Bag-of-Words and Data Augmentation
%text: Impact of Parallel vs. Non Parallel Corpora on the Identification of Arabic Dialects
%speech: Multi-Scale Channel Adaptive Time-Delay Neural Network and Balanced Fine-Tuning for Arabic Dialect Identification
%speech: Dialect classification using acoustic and linguistic features in Arabic speech
%======================== MT ==============================
%Alongside these efforts, 
%were dedicated towards the task of DA-MSA translation. 
% OSACT Shared task, outline main approaches (including: LLM-based MT Data Creation: Dialectal to MSA Translation Shared Task and AraT5-MSAizer)
% Anastasopoulos et al. (https://arxiv.org/pdf/2305.17267)
% Other efforts have focused on one dialect, including Egyptian, Tunisian, and Algerian dialects.
% More efforts on Arabic/Foreign MT:
% - SOTA review paper: https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=10233872 and https://ieeexplore.ieee.org/abstract/document/10469415 
%, where recent litersture overviews on the latter translation task can be found in \cite{literature_reviews}. 
% - relevant datasets
% - Several benchmarks on LLMs involving Ar-> Foreign rather than between Arabic variants: QCRI's paper, DOLPHIN, Hopkins et al. (https://arxiv.org/pdf/2404.13813)
% - Also, work on En-to-Ar: 
% --- https://ieeexplore.ieee.org/document/10330525
% ---- Error Analysis on PLMs En-to-Ar MT (https://link.springer.com/article/10.1007/s44230-024-00061-7)
% - Also, relevant work to dialectal Arabic translation included:
% --- Unveiling the New Frontier: ChatGPT-3 Powered Translation for Arabic-English Language Pairs
% --- Abdul-Mageed's paper: Interplay of Machine Translation, Diacritics, and Diacritization (Doesn't involve Arabic)
% - Sennrich's paper on evaluation metrics for dialects with unstandardized orthography (https://arxiv.org/pdf/2311.16865)
% - (little work on CSW MT: DOLHPIN, Hamed et al.)

==> table/subtask1_full_results.tex <==
\begin{table*}[tb]
    \aboverulesep=0ex % Solution part 1 of 3
    % \belowrulesep=0ex % Solution part 1 of 3
    % \rule{0pt}{1EM}% Solution part 2 of 3 (% is required)
    \centering
    \small
        \begin{tabular}{cl|ccccccccc|c}
        \multirow{2}{*}{\textbf{Rk}}&\multirow{2}{*}{\textbf{System}} & \multicolumn{9}{c}{\textbf{F1-score (per country)}} & \textbf{Macro Avg.}\\
        &&  \multirow{1}{*}{\textbf{Algeria}} &  \multirow{1}{*}{\textbf{Egypt}} &  \multirow{1}{*}{\textbf{Iraq}} &  \multirow{1}{*}{\textbf{Morocco}} &  \multirow{1}{*}{\textbf{Palestine}} &  \multirow{1}{*}{\textbf{Sudan}} &  \multirow{1}{*}{\textbf{Syria}} &  \multirow{1}{*}{\textbf{Tunisia}} &  \multirow{1}{*}{\textbf{Yemen}} &  \textbf{F1-score ($\uparrow$)} \\
        \midrule
        \textcolor{blue}{Baseline I}&Top 90\%&    49.30 &  71.70 & 57.36 &    59.64 &      58.16 &  55.27 &  46.60 &    56.77 &  52.95 &             56.42 \\
        % top4 &    54.58 &  66.67 & 55.14 &    61.50 &      52.56 &  55.25 &  54.06 &    49.25 &  49.69 &             55.41 \\
        % top5 &    52.88 &  64.69 & 55.17 &    61.89 &      53.51 &  56.57 &  56.37 &    45.09 &  52.19 &             55.37 \\
        % top3 &    55.20 &  66.67 & 55.06 &    62.43 &      54.31 &  53.36 &  48.47 &    53.03 &  47.28 &             55.09 \\
        % \textcolor{blue}{Baseline II}&top2 &    50.91 &  67.81 & 54.40 &    60.98 &      54.21 &  49.41 &  40.85 &    59.06 &  42.32 &             53.33 \\
        1&\textbf{Elyadata} &    47.58 &  60.46 & 45.61 &    42.54 &      55.15 &  53.97 &  55.64 &    37.64 &  56.57 &             50.57 \\
        \textcolor{blue}{Baseline II} & Top 1 &    42.24 &  65.62 & 53.45 &    57.89 &      45.47 &  46.25 &  33.98 &    58.91 &  35.15 &             48.77 \\
        2&\textbf{NLP\_DI } &    42.59 &  62.11 & 36.98 &    32.08 &      55.59 &  38.67 &  42.12 &    33.33 &  45.97 &             43.27 \\
        \textcolor{blue}{Baseline III} & Random &    34.34 &  38.61 & 33.11 &    29.34 &      37.30 &  41.78 &  48.81 &    25.25 &  45.86 &             37.15 \\
        % geo &    27.03 &  33.60 & 34.73 &    31.91 &      29.24 &  28.91 &  23.69 &    31.80 &  23.61 &             29.39 \\
        3&\textbf{dzNlp} &    15.84 &  32.51 & 20.91 &    21.97 &      25.62 &  18.14 &  16.67 &    21.62 &  15.52 &             20.98 \\
        \bottomrule
        \end{tabular}
    \caption{Performance of the systems on the test set of Subtask \#1.}
    \label{tab:subtask1_f1_detailed}
\end{table*}


==> table/subtask1_results_v2.tex <==
\begin{table}[tb]
    \centering
    %\setlength{\tabcolsep}{3pt}
\resizebox{\columnwidth}{!}{%
    \begin{tabular}{clcccc}
    \toprule
        \multirow{2}{*}{\textbf{Rk}}& \multirow{2}{*}{\textbf{System}} & \multicolumn{4}{c}{\textbf{Macro-average}}\\ \cmidrule{3-6}
        %& & \textbf{Accuracy ($\uparrow$)}& \textbf{Precision ($\uparrow$)}& \textbf{Recall ($\uparrow$)}& \textbf{\texttt{F\textsubscript{1}} score ($\uparrow$)}\\
        & & \textbf{A ($\uparrow$)}& \textbf{P ($\uparrow$)}& \textbf{R ($\uparrow$)}& \textbf{\texttt{F\textsubscript{1}}($\uparrow$)}\\
        \midrule
            \textcolor{blue}{Baseline I}& \multirow{1}{*}{Top 90\%} & \textbf{78.7\textsubscript{±6.2}} & 74.9\textsubscript{±8.3} & 46.8\textsubscript{±10.2} & \textbf{56.4\textsubscript{±6.7}}\\ \cdashline{1-6}
            1 & \multirow{1}{*}{\textbf{Elyadata}} & 67.5\textsubscript{±3.7} & 46.5\textsubscript{±10.1} & \textbf{57.1\textsubscript{±5.1}} & 50.6\textsubscript{±7.1}\\\cdashline{1-6}
            \textcolor{blue}{Baseline II}& \multirow{1}{*}{Top 1} & 78.2\textsubscript{±7.8} & \textbf{86.8\textsubscript{±6.5}} & 34.9\textsubscript{±10.2} & 48.8\textsubscript{±10.3}\\ \cdashline{1-6}
            2& \multirow{1}{*}{\textbf{NLP\_DI}} & 71.9\textsubscript{±5.6} & 53.6\textsubscript{±10.2} & 37.4\textsubscript{±11.0} & 43.3\textsubscript{±9.4}\\ \cdashline{1-6}
            \textcolor{blue}{Baseline III}& \multirow{1}{*}{Random} & 50.1\textsubscript{±1.6} & 30.4\textsubscript{±8.8} & 50.2\textsubscript{±2.1} & 37.2\textsubscript{±7.2}\\ \cdashline{1-6}
            3 & \multirow{1}{*}{\textbf{dzNlp}} & 71.4\textsubscript{±7.2} & 63.2\textsubscript{±10.7} & 12.9\textsubscript{±3.8} & 21.0\textsubscript{±5.2}\\

        \bottomrule
    \end{tabular}%
    }
    
    \caption{
    Performance of the systems on the test set of Subtask~1, showing accuracy (A), Precision (P), Recall (R) and \texttt{F\textsubscript{1}} score (\texttt{F\textsubscript{1}}). Results are sorted by \texttt{F\textsubscript{1}} score.}
    \label{tab:subtask1_f1}
\end{table}

==> table/subtasks_results.tex <==
\begin{table}[tb]

% \begin{subtable}[c]{0.6\textwidth}
% \scriptsize
% \centering
% \input{table/subtask1_results}
% \subcaption{Subtask 1 - MDLID}
% \label{tab:subtask1_f1}
% \end{subtable}
% ~
% \begin{subtable}[c]{0.3\textwidth}
% \scriptsize
% \centering
% \input{table/subtask2_results}
% \subcaption{Subtask 2 - ALDi Estimation}
% \label{tab:subtask2_RMSE_test}
% \end{subtable}

% \begin{subtable}[c]{\textwidth}
% \scriptsize
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{clccccc@{}}
\toprule
% \textbf{Rk} & \multicolumn{1}{c}{\textbf{Team}} & \textbf{Overall} & \textbf{Egyptain} & \textbf{Emirati} & \textbf{Jordanian} & \textbf{Palestinian} \\ \midrule
\textbf{Rank} & \multicolumn{1}{c}{\textbf{Team}} & \multicolumn{1}{c}{\textbf{Overall}} & \multicolumn{1}{c}{\textbf{Egy.}} & \multicolumn{1}{c}{\textbf{Emi.}} & \multicolumn{1}{c}{\textbf{Jor.}} & \multicolumn{1}{c}{\textbf{Pal.}} \\ \midrule
1 & Arabic Train             & 20.44  & 18.74   & 12.47  & 16.46    & 17.22      \\
2  & Alson                    & 17.46  & 16.53   & 15.23  & 17.12    & 18.24      \\
3  &  ASOS                     & 17.13  & 16.66   & 12.80  & 14.87    & 16.05      \\
4 &  CUFE                     & 16.09  & 15.04   & 13.34  & 14.50    & 16.31      \\
5  &  MBZUAI BLEU              & 10.54  &  8.69   &  8.00  &  8.40    & 10.08      \\

6 &  VBNN                     &  9.24  & 10.58   &  8.43  & 11.51    &  9.35      \\
\multicolumn{1}{l}{\textcolor{blue}{Baseline I}}            &   AraT5\textsubscript{v2}  &  6.87  &  9.38  &  4.61  & 4.90 &  8.13    \\

7 &  MBZUAI BADG              &  2.78  &  3.51   &  2.05  &  2.84    &  2.64      \\
\multicolumn{1}{l}{\textcolor{blue}{Baseline II}}             & mT5 & 2.81  &  3.08  &  2.23  &  3.11  &  2.95    \\


\multicolumn{1}{l}{\textcolor{blue}{Baseline III}}        & AraBART &0.87  &  0.77  &  0.81  &  1.11  &  0.88     \\
8 &  Shaheen                  & 0.00   & 0.00    &  0.00  &  0.00    &  0.00      \\ 


   % \cdashline{1-7}


\bottomrule
\end{tabular}%
}
% \subcaption{Subtask 3 - DA to MSA Translation}
% \end{subtable}
\caption{Subtask 3 - DA to MSA Translation}
\label{tab:subtask3_res}
% \end{subtable}
% \caption{The performance of the different systems on the test sets of the three subtasks.}


\end{table}
